MeetSense: A Lightweight Framework for Group Identification using Smartphones

In an organization, individuals prefer to form various formal and informal groups for mutual interactions. Therefore, ubiquitous identification of such groups and understanding their dynamics are important to monitor activities, behaviours and well-being of the individuals. In this paper, we develop a lightweight, yet near-accurate, methodology, called MeetSense, to identify various interacting groups based on collective sensing through users' smartphones. Group detection from sensor signals is not straightforward because users in proximity may not always be under the same group. Therefore, we use acoustic context extracted from audio signals to infer interaction pattern among the subjects in proximity. We have developed an unsupervised and lightweight mechanism for user group detection by taking cues from network science and measuring the cohesivity of the detected groups in terms of modularity. Taking modularity into consideration, MeetSense can efficiently eliminate incorrect groups, as well as adapt the mechanism depending on the role played by the proximity and the acoustic context in a specific scenario. The proposed method has been implemented and tested under many real-life scenarios in an academic institute environment, and we observe that MeetSense can identify user groups with close to 90% accuracy even in a noisy environment.

==> tex/2_related_works.tex <==
\section{Related Works} \label{rwo}
The naive way for continuous tracking of various user groups in the vicinity is the video surveillance based systems~\cite{zhang2015tracking}. However, such systems require deployment of fixed video capturing infrastructures even at the informal meeting places, such as cafeterias. In this line, several applications such as  emergency control \cite{gordon2012group}, public safety management \cite{du2016group}, 
student life management \cite{wang2014studentlife}, student performance management \cite{agrawal2014grouping}, organizational behavior measurement \cite{olguin2009sensible} and context sharing \cite{lee2012comon,lee2016comon+} etc. utilize various wearables \cite{olguin2009sensible} and smartphones \cite{sen2014} to capture the interaction as well as the overall structure of the group information. Recent literatures admit that the definition of a group varies with its utility purpose. For example, in \cite{olguin2009sensible}, the authors described an automatic organizational behaviour monitoring system, whereas \cite{lee2012comon} developed a novel cooperative context monitoring system by opportunistically detecting the cooperators among nearby devices. Besides the applications, a few works \cite{gordon2012group,olguin2009sensible,lee2012comon,kar63969} acknowledge the importance of data tracking devices in the context of group detection. Olguin \emph{et al.} \cite{olguin2009sensible} measured face-to-face interaction, physical proximity and physical activity levels using sociometric badge \cite{olguin2006wearable}. Gordon \emph{et al.} \cite{gordon2013towards} introduced coffee mugs \cite{gordon2012group} for recognizing the group activities like meeting, presentation, etc. among the users. However, the target participants these specific groups based on wearables are closed and requires specific devices acquisitions, whereas the off-the-shelf commodity smartphones cross the hurdle of participant count. Towards this line, Du \emph{et al.} \cite{du2016group} discussed the group structure and mobility patterns using smartphone usage characteristics. In \cite{kar63969}, the authors utilized smartphones for meeting group identification, which is the prime objective of this paper. Henceforth, we move forward to discuss the various sensing medium present in the smartphone for detecting meeting groups.

\textbf{Sensing medium based group study:}
In the current era, smartphones comprise with multiple numbers of sensors. Each sensor has its capacity and limitations for sensing the context of the group members in the targeted application. Considering the instance of proximity detection model, outdoor context is highly dominated by GPS whereas, in indoor context, GPS performs poorly \cite{radu2014semi}. Depending upon the sensing type, the popular approaches in this context can be divided into two categories -- (1) \textit{Proximity sensing} and (2) \textit{User Interaction measurements}, which are useful in the context of user group identification. 
%The former category includes location, in which Bluetooth \cite{do2011groupus}, WiFi \cite{sen2014}, and GPS \cite{casagranda2015audio} sense the proximity information to infer the group whereas the later considers microphone \cite{casagranda2015audio} accelerometer \cite{du2016group}, magnetometer \cite{wang2012no}, light \cite{azizyan2009surroundsense}, barometer \cite{sen2014} etc. to sense the surroundings to observe the group. 

\textit{Proximity Sensing:} GPS is a well-known system for localizing the object. Casagranda \emph{et al.} explored the GPS based proximity information for detecting the group~\cite{casagranda2015audio} . However in indoor scenarios, capturing proximity only with GPS is challenging due to the low coverage \cite{chintalapudi2010indoor}. Bluetooth is another existing technology used for estimating the proximity information of users~\cite{do2011groupus}. Liu \emph{et al.} highlighted the Bluetooth high coverage property in both indoor and outdoor environment \cite{liu2014face} and provided a compelling alternative for proximity estimation. In \cite{lee2016comon+}, Lee \emph{et al.} used the Bluetooth to sense the nearby devices for developing a cooperative context monitoring system. On the contrary, Friedman \emph{et al.} \cite{friedman2013power} identified the superiority of WiFi on top of Bluetooth. Several works \cite{chintalapudi2010indoor,azizyan2009surroundsense,wang2012no,abdelnasser2016semanticslam,hong2016socialprobe,sugasaki2017robust,wu2017gain} have been done on indoor localization based on the WiFi sensed proximity information. In \cite{sapiezynski2017}, the authors worked with WiFi fingerprint to infer the proximity information in a supervised manner. On the other hand, the authors in~\cite{wang2012no,kar63969} developed unsupervised approaches for inferring proximity based on WiFi signal strength.

%\textit{Audio, Inertial and Others:} 
\textit{User Interaction Measurements:} A number of works has utilized different smartphone sensors for understanding the environmental context and interaction patterns. The microphone is one important medium for sensing the environmental context \cite{azizyan2009surroundsense}. Lee \emph{et al.} \cite{lee2013sociophone} introduced a supervised microphone data-based system for monitoring face to face interaction. The supervised scheme was replaced by unsupervised approaches for similar applications in \cite{casagranda2015audio,kar63969}. Alameda-Pineda \emph{et al.} \cite{alameda2015analyzing} introduced an alternative solution for analyzing the free-standing conversational group by head and body pose estimation using audio and infrared signals. The inertial sensors are mainly explored to identify user-specific or environment specific characteristics for improving the accuracy of the overall group detection system. Towards this direction, Sen \emph{et al.} \cite{sen2014} used the accelerometer and compass, and barometer data for detecting similarity in the motion, turns, and levels, respectively. In \cite{azizyan2009surroundsense}, the authors explored the light information tor sense the surroundings. 

\begin{table*}
	\centering
	\caption{Different Group Schemes and Respective Detection Mechanisms with Parameter Metrics}
	\label{relwork}
	\begin{tabular}{|l|l|l|l|l|l|}
		\hline
		\multicolumn{1}{|c|}{\textbf{Group Schemes}} & \multicolumn{1}{c|}{\textbf{Used Sensors}}                                         & \multicolumn{1}{c|}{\textbf{Supervised?}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Indoor/\\ Outdoor?\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Static/\\ Motion?\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Noise\\ Tolerance \end{tabular}}} \\ \hline
		SocialProbe \cite{hong2016socialprobe}                                 & Passive WiFi                                                                       & No                                        & Indoor                                                                                   & Both                                                                                               & Low                                                                                             \\ \hline
		AudioMatch \cite{casagranda2015audio}                                  & GPS, Microphone                                                                    & No                                        & Both                                                                                     & Both                                                                                               & Low                                                                                             \\ \hline
		GruMon \cite{sen2014}                                      & \begin{tabular}[c]{@{}l@{}}WiFi, Accelerometer, \\ Compass, Barometer\end{tabular} & Yes                                       & Indoor                                                                                   & Motion                                                                                             & Medium                                                                                          \\ \hline
		Next2Me \cite{kar63969}                                     & WiFi, Microphone                                                                   & No                                        & Indoor                                                                                   & Static                                                                                             & Low                                                                                             \\ \hline
		\textbf{GroupSense} (This paper)                         & WiFi, Microphone                                                                   & No                                        & Both                                                                                     & Both                                                                                               & Medium                                                                                          \\ \hline
	\end{tabular}
\end{table*}

\textbf{Summary:}
Although a number of works in the existing literature has studied capturing proximity and environmental context from various smartphone and wearable sensors, a few of them studies the problem of user group identification from such contextual informations~\cite{hong2016socialprobe,casagranda2015audio,sen2014,kar63969} . A comparative study between the current state of the art works and the proposed group detection mechanisms is shown in Table \ref{relwork}. Different applications interpret groups differently. Similarly, different systems are also developed for different types of groups. We observe that various studies in the literature for inferring user groups can be classified based on four major parameters -- (a) detection mechanism (supervised or unsupervised), (b) environment (indoor or outdoor), (c) mobility support (static or mobile groups) and (d) noise tolerance level. Although the majority of the works focus on the group identification in the indoor environment, a few works consider outdoor and mobile scenarios for group detection. Moreover, the experimental results demonstrate that the existing group detection methodologies are either capable of handling pre-assumed white and pink noises or noise in the controlled environment. However, none of the work considers unsupervised, indoor-outdoor bound-free, static-motion constraint-free, and dominant noise system. Nevertheless, the existing works mostly focus on group identification where the user carries similar types of devices.  
 


==> tex/6a_baseline2.tex <==
\subsection{Baseline2 - GruMon}
GruMon \cite{sen2014} is a real-time group monitoring system for urban spaces leveraging on the location, motion, turn, and level of the members. More specifically, the system computes similarity values of WiFi, accelerometer, compass, and barometer readings for measuring the membership of a group. The location similarity is calculated using a pre-collected fingerprint map and hyperbolic Radar. As we mentioned earlier, we do not have any pre-knowledge of the location. Therefore, we are unable to use such fingerprint-based system. Hence, we replace the location feature computation of GruMon by our Joint Jaccard and Gain measure. Additionally, in our application scenarios, as turn and level of the members do not impact much on the group formation, we have not tracked the compass and barometer data. Hence, we are compromising these two features for GruMon implementation. Although we are not using accelerometer signature for our model \textit{GroupSense}, we compute the motion feature using the decision tree as described in GruMon \cite{sen2014}}. Finally, the weighted location and motion features are placed to the binary SVM classifier for filtering out the non-group pairing information followed by Markov Cluster algorithm for detecting the group.  
